Denoising Architecture for Unsupervised Anomaly Detection in Time-Series

Anomalies in time-series provide insights of critical scenarios across a range of industries, from banking and aerospace to information technology, security, and medicine. However, identifying anomalies in time-series data is particularly challenging due to the imprecise definition of anomalies, the frequent absence of labels, and the enormously complex temporal correlations present in such data. The LSTM Autoencoder is an Encoder-Decoder scheme for Anomaly Detection based on Long Short Term Memory Networks that learns to reconstruct time-series behavior and then uses reconstruction error to identify abnormalities. We introduce the Denoising Architecture as a complement to this LSTM Encoder-Decoder model and investigate its effect on real-world as well as artificially generated datasets. We demonstrate that the proposed architecture increases both the accuracy and the training speed, thereby, making the LSTM Autoencoder more efficient for unsupervised anomaly detection tasks.

==> Backup.tex <==
\begin{table}[t]

\caption{Experiments results2}\label{tab:expirements_results2}
\centering
\begin{tabular}{|c|cccccc|}
\hline
Dataset &
  \multicolumn{1}{c|}{Arch} &
  \multicolumn{1}{c|}{Dropout} &
  \multicolumn{1}{c|}{Epochs} &
  \multicolumn{1}{c|}{Recall} &
  \multicolumn{1}{c|}{Precision} &
  F1 \\ \hline
   &
   &
  0.0 &
  29 &
  0.198542 &
  0.442812 &
  0.274159 \\
 &
   &
  0.1 &
  14 &
  0.199482 &
  0.444911 &
  0.275459 \\
 &
   &
  0.2 &
  18 &
  0.205363 &
  0.457787 &
  0.283534 \\
 &
   &
  0.3 &
  18 &
  0.216184 &
  0.481656 &
  0.298425 \\
 &
   &
  \cellcolor[HTML]{C7FAC6}0.4 &
  \cellcolor[HTML]{C7FAC6}9 &
  \cellcolor[HTML]{C7FAC6}0.219948 &
  \cellcolor[HTML]{C7FAC6}0.490814 &
  \cellcolor[HTML]{C7FAC6}0.303769 \\
 &
  \multirow{-6}{*}{16} &
  0.5 &
  9 &
  0.217596 &
  0.485310 &
  0.300471 \\ \cline{2-7} 
  
   &
   &
  0.0 &
  18 &
  0.194778 &
  0.434190 &
  0.268918 \\
 &
   &
  0.1 &
  27 &
  0.209598 &
  0.466981 &
  0.289333 \\
 &
   &
  0.2 &
  11 &
  0.214067 &
  0.477189 &
  0.295551 \\
 &
   &
  0.3 &
  7 &
  0.220654 &
  0.492130 &
  0.304694 \\
 &
   &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 0.4} &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 7} &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 0.231475} &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 0.516535} &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 0.319688} \\
\multirow{-12}{*}{A1} &
  \multirow{-6}{*}{16, 8} &
  0.5 &
  14 &
  0.218772 &
  0.487933 &
  0.302095 \\ \hline
  \end{tabular}%
  \hspace{1cm}%
\begin{tabular}{|c|cccccc|}
\hline
Dataset &
  \multicolumn{1}{c|}{Arch} &
  \multicolumn{1}{c|}{Dropout} &
  \multicolumn{1}{c|}{Epochs} &
  \multicolumn{1}{c|}{Recall} &
  \multicolumn{1}{c|}{Precision} &
  F1 \\ \hline
   &
   &
  0.0 &
  21 &
  1.000000 &
  0.597741 &
  0.748233 \\
 &
   &
  0.1 &
  9 &
  1.000000 &
  0.597222 &
  0.747826 \\
 &
   &
  \cellcolor[HTML]{FFFFC7}0.2 &
  \cellcolor[HTML]{FFFFC7}10 &
  \cellcolor[HTML]{FFFFC7}1.000000 &
  \cellcolor[HTML]{FFFFC7}0.597568 &
  \cellcolor[HTML]{FFFFC7}0.748097 \\
 &
   &
  0.3 &
  18 &
  1.000000 &
  0.597568 &
  0.748097 \\
 &
   &
  0.4 &
  10 &
  0.990795 &
  0.591896 &
  0.741076 \\
 &
  \multirow{-6}{*}{16} &
  0.5 &
  9 &
  0.946221 &
  0.565268 &
  0.707737 \\ \cline{2-7} 
 &
   &
  0.0 &
  24 &
  1.000000 &
  0.597741 &
  0.748233 \\
 &
   &
  \cellcolor[HTML]{FFFFC7}0.1 &
  \cellcolor[HTML]{FFFFC7}15 &
  \cellcolor[HTML]{FFFFC7}1.000000 &
  \cellcolor[HTML]{FFFFC7}0.597222 &
  \cellcolor[HTML]{FFFFC7}0.747826 \\
 &
   &
  0.2 &
  12 &
  0.998062 &
  0.596583 &
  0.746783 \\
 &
   &
  0.3 &
  9 &
  0.928779 &
  0.555169 &
  0.694943 \\
 &
   &
  0.4 &
  14 &
  0.816376 &
  0.487699 &
  0.610618 \\
\multirow{-12}{*}{A3} &
  \multirow{-6}{*}{16, 8} &
  0.5 &
  14 &
  0.837209 &
  0.500000 &
  0.626087 \\ \hline
  \end{tabular}
\begin{tabular}{|c|cccccc|}
\hline
Dataset &
  \multicolumn{1}{c|}{Arch} &
  \multicolumn{1}{c|}{Dropout} &
  \multicolumn{1}{c|}{Epochs} &
  \multicolumn{1}{c|}{Recall} &
  \multicolumn{1}{c|}{Precision} &
  F1 \\ \hline
   &
   &
     0.0 &
  22 &
  1.000000 &
  0.401042 &
  0.572491 \\
 &
   &
  0.1 &
  11 &
  1.000000 &
  0.401042 &
  0.572491 \\
 &
   &
  \cellcolor[HTML]{FFFFC7}0.2 &
  \cellcolor[HTML]{FFFFC7}7 &
  \cellcolor[HTML]{FFFFC7}1.000000 &
  \cellcolor[HTML]{FFFFC7}0.401042 &
  \cellcolor[HTML]{FFFFC7}0.572491 \\
 &
   &
  0.3 &
  7 &
  1.000000 &
  0.401158 &
  0.572609 \\
 &
   &
  0.4 &
  10 &
  1.000000 &
  0.401042 &
  0.572491 \\
 &
  \multirow{-6}{*}{16} &
  0.5 &
  11 &
  1.000000 &
  0.401158 &
  0.572609 \\ \cline{2-7} 
 &
   &
  0.0 &
  23 &
  1.000000 &
  0.401390 &
  0.572846 \\
 &
   &
  0.1 &
  7 &
  1.000000 &
  0.401042 &
  0.572491 \\
 &
   &
  \cellcolor[HTML]{FFFFC7}0.2 &
  \cellcolor[HTML]{FFFFC7}12 &
  \cellcolor[HTML]{FFFFC7}1.000000 &
  \cellcolor[HTML]{FFFFC7}0.401274 &
  \cellcolor[HTML]{FFFFC7}0.572727 \\
 &
   &
  0.3 &
  14 &
  0.997114 &
  0.400116 &
  0.571074 \\
 &
   &
  0.4 &
  17 &
  0.994228 &
  0.398727 &
  0.569186 \\
\multirow{-12}{*}{A4} &
  \multirow{-6}{*}{16, 8} &
  0.5 &
  17 &
  0.805195 &
  0.323104 &
  0.461157 \\ \hline
 \end{tabular}
\end{table}




\begin{table}[t]
\caption{Experiments results}\label{tab:expirements_results}
\centering
\begin{tabular}{|c|cccccc|}
\hline
Dataset &
  \multicolumn{1}{c|}{Architecture} &
  \multicolumn{1}{c|}{Dropout} &
  \multicolumn{1}{c|}{Epochs} &
  \multicolumn{1}{c|}{Recall} &
  \multicolumn{1}{c|}{Precision} &
  F1-Score \\ \hline
 &
   &
  0.0 &
  29 &
  0.198542 &
  0.442812 &
  0.274159 \\
 &
   &
  0.1 &
  14 &
  0.199482 &
  0.444911 &
  0.275459 \\
 &
   &
  0.2 &
  18 &
  0.205363 &
  0.457787 &
  0.283534 \\
 &
   &
  0.3 &
  18 &
  0.216184 &
  0.481656 &
  0.298425 \\
 &
   &
  \cellcolor[HTML]{C7FAC6}0.4 &
  \cellcolor[HTML]{C7FAC6}9 &
  \cellcolor[HTML]{C7FAC6}0.219948 &
  \cellcolor[HTML]{C7FAC6}0.490814 &
  \cellcolor[HTML]{C7FAC6}0.303769 \\
 &
  \multirow{-6}{*}{16} &
  0.5 &
  9 &
  0.217596 &
  0.485310 &
  0.300471 \\ \cline{2-7} 
 &
   &
  0.0 &
  18 &
  0.194778 &
  0.434190 &
  0.268918 \\
 &
   &
  0.1 &
  27 &
  0.209598 &
  0.466981 &
  0.289333 \\
 &
   &
  0.2 &
  11 &
  0.214067 &
  0.477189 &
  0.295551 \\
 &
   &
  0.3 &
  7 &
  0.220654 &
  0.492130 &
  0.304694 \\
 &
   &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 0.4} &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 7} &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 0.231475} &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 0.516535} &
  \cellcolor[HTML]{C7FAC6}{\color[HTML]{333333} 0.319688} \\
\multirow{-12}{*}{A1} &
  \multirow{-6}{*}{16, 8} &
  0.5 &
  14 &
  0.218772 &
  0.487933 &
  0.302095 \\ \hline
 &
   &
  0.0 &
  21 &
  1.000000 &
  0.597741 &
  0.748233 \\
 &
   &
  0.1 &
  9 &
  1.000000 &
  0.597222 &
  0.747826 \\
 &
   &
  \cellcolor[HTML]{FFFFC7}0.2 &
  \cellcolor[HTML]{FFFFC7}10 &
  \cellcolor[HTML]{FFFFC7}1.000000 &
  \cellcolor[HTML]{FFFFC7}0.597568 &
  \cellcolor[HTML]{FFFFC7}0.748097 \\
 &
   &
  0.3 &
  18 &
  1.000000 &
  0.597568 &
  0.748097 \\
 &
   &
  0.4 &
  10 &
  0.990795 &
  0.591896 &
  0.741076 \\
 &
  \multirow{-6}{*}{16} &
  0.5 &
  9 &
  0.946221 &
  0.565268 &
  0.707737 \\ \cline{2-7} 
 &
   &
  0.0 &
  24 &
  1.000000 &
  0.597741 &
  0.748233 \\
 &
   &
  \cellcolor[HTML]{FFFFC7}0.1 &
  \cellcolor[HTML]{FFFFC7}15 &
  \cellcolor[HTML]{FFFFC7}1.000000 &
  \cellcolor[HTML]{FFFFC7}0.597222 &
  \cellcolor[HTML]{FFFFC7}0.747826 \\
 &
   &
  0.2 &
  12 &
  0.998062 &
  0.596583 &
  0.746783 \\
 &
   &
  0.3 &
  9 &
  0.928779 &
  0.555169 &
  0.694943 \\
 &
   &
  0.4 &
  14 &
  0.816376 &
  0.487699 &
  0.610618 \\
\multirow{-12}{*}{A3} &
  \multirow{-6}{*}{16, 8} &
  0.5 &
  14 &
  0.837209 &
  0.500000 &
  0.626087 \\ \hline
 &
   &
  0.0 &
  22 &
  1.000000 &
  0.401042 &
  0.572491 \\
 &
   &
  0.1 &
  11 &
  1.000000 &
  0.401042 &
  0.572491 \\
 &
   &
  \cellcolor[HTML]{FFFFC7}0.2 &
  \cellcolor[HTML]{FFFFC7}7 &
  \cellcolor[HTML]{FFFFC7}1.000000 &
  \cellcolor[HTML]{FFFFC7}0.401042 &
  \cellcolor[HTML]{FFFFC7}0.572491 \\
 &
   &
  0.3 &
  7 &
  1.000000 &
  0.401158 &
  0.572609 \\
 &
   &
  0.4 &
  10 &
  1.000000 &
  0.401042 &
  0.572491 \\
 &
  \multirow{-6}{*}{16} &
  0.5 &
  11 &
  1.000000 &
  0.401158 &
  0.572609 \\ \cline{2-7} 
 &
   &
  0.0 &
  23 &
  1.000000 &
  0.401390 &
  0.572846 \\
 &
   &
  0.1 &
  7 &
  1.000000 &
  0.401042 &
  0.572491 \\
 &
   &
  \cellcolor[HTML]{FFFFC7}0.2 &
  \cellcolor[HTML]{FFFFC7}12 &
  \cellcolor[HTML]{FFFFC7}1.000000 &
  \cellcolor[HTML]{FFFFC7}0.401274 &
  \cellcolor[HTML]{FFFFC7}0.572727 \\
 &
   &
  0.3 &
  14 &
  0.997114 &
  0.400116 &
  0.571074 \\
 &
   &
  0.4 &
  17 &
  0.994228 &
  0.398727 &
  0.569186 \\
\multirow{-12}{*}{A4} &
  \multirow{-6}{*}{16, 8} &
  0.5 &
  17 &
  0.805195 &
  0.323104 &
  0.461157 \\ \hline
\end{tabular}%
\end{table}
